Can Large Language Models be Good Path Planners? A Benchmark and Investigation on Spatial-temporal Reasoning

Large language models (LLMs) have achieved remarkable success across a wide spectrum of tasks; however, they still face limitations in scenarios that demand long-term planning and spatial reasoning. To facilitate this line of research, in this work, we propose a new benchmark, termed $\textbf{P}$ath $\textbf{P}$lanning from $\textbf{N}$atural $\textbf{L}$anguage ($\textbf{PPNL}$). Our benchmark evaluates LLMs' spatial-temporal reasoning by formulating ''path planning'' tasks that require an LLM to navigate to target locations while avoiding obstacles and adhering to constraints. Leveraging this benchmark, we systematically investigate LLMs including GPT-4 via different few-shot prompting methodologies as well as BART and T5 of various sizes via fine-tuning. Our experimental results show the promise of few-shot GPT-4 in spatial reasoning, when it is prompted to reason and act interleavedly, although it still fails to perform long-term temporal reasoning. In contrast, while fine-tuned LLMs achieved impressive results on in-distribution reasoning tasks, they struggled to generalize to larger environments or environments with more obstacles.

==> iclr2023/sec_benchmark.tex <==

\section{Benchmark Overview}\label{sec:benchmark}

\subsection{Tasks Formulation}

\textbf{Path Planning:} Formally, we describe the problem as follows: given a set of $l$ location $P = \{P_0, P_1, ..., P_l\}$, a set of $k$ obstacles $O = \{O_0, O_1, ..., O_k\}$ and a constraint $C$, the task is provide a sequence of actions $A = \{A_0, A_1, ..., A_t\}$ such that $\{ L(i) \neq O_j  \forall 0 \leq i \leq t, 0 \leq j \leq k \}$ and $A$ satisfies $C$, where $L(i)$ is the position of the agent at after performing action $A_i$.    


\textbf{Settings: } We explore this problem on $N \times N$ grids. The settings that we consider are the following: 
\begin{enumerate}[noitemsep, nolistsep]
    \item \textbf{Single-goal setting}: the task is to visit a single goal location.
    \item \textbf{Multi-goal settings}: the task is to reach multiple goal locations. In this case, we distinguish two different types of settings: (1) \textbf{No Constraints}: where the task is simply to visit all goal locations, (2) \textbf{Constrained Ordering}, where a set of goal locations has to be visited before others.
    
\end{enumerate}  


\textbf{Tasks: } In Section~\ref{datagen}, we will introduce the details for generating different environments (i.e. grids with different obstacle placements) as well as initial and goal placements (i.e., a specific task environment with specified initial and target locations) under different settings. We consider three different generalization tests:
\begin{enumerate}[noitemsep, nolistsep]
    \item In-distribution generalization involving testing the ability to generalize to familiar grid environments with matching sizes and obstacle counts.
    \item   Generalization to varied environment sizes, where we assess how well the models perform in grid environments of different sizes from their training data.  
    \item Generalization to worlds with more obstacles, where we evaluate the ability of the models to navigate environments containing a larger number of obstacles than the environments used for training.
\end{enumerate}

\subsection{Data Generation Process}\label{datagen}

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{iclr2023/figures/PPNL.png}
  \caption{Overview of the data generation process.}
  \label{fig:datagen}
\end{figure}

Figure \ref{fig:datagen} provides an overview of the process we followed in order to generate our synthetic dataset. We first begin by generating environments for both in-distribution and out-of-distribution evaluation; we then place the agent and the different goals in each of these environment and map each one of these queries with an optimal path and a natural language description. This section provides a more detailed description of this process. 

\textbf{Environments Generation: } For the in-distribution set, we sample 836 6x6 grids with obstacles ranging with random arrangements of 1-5 obstacles. We reserve 80\% of these environments for training while the remaining 168 are used for testing. We also generate three out-of-distribution sets consisting of: larger grids (7x7), smaller grids (5x5) and more obstacles (6-11 Obstacles). For each of these test sets, We generate 25 environments corresponding to each number of obstacles. Hence, in total, the test sets consisting of 7x7 and 5x5 grids encompass 125 environments, while the test set with 6-11 obstacles is made up of 150 environments.


\textbf{Agent and Goals Placement: } We provide the different samples in our dataset by randomly drawing different placements for the agent and and goals for each environment in Table \ref{tab:overall-stats}. 

\begin{itemize}[noitemsep, nolistsep]
    \item \textit{Single-goal Setting:}  For the single-goal setting, we sample 30 random start and goal positions from each environment. Within each environments we only use 80\% (24) of the placements for training, and reserve 10\% (3) for development and another 10\% (3) for a separate test set consisting of unseen placements as we also wanted to look at whether the models are able to generalize to novel start-goal combinations within environments that have been encountered in training. 
    \item \textit{Multi-goal Setting:} Similarly, for the multi-goal setting, for each environment, we sample 10 random arrangements of a starting position and a each number of goals in the range [2, 6]. For each arrangement, we consider a task setting without constraints and with a randomly chosen ordering constraint. We also only use 80\% (8) of the placements for training, and reserve 10\% (1) and another 10\% (1) for testing. A breakdown of the overall data statistics by in Table \ref{tab:overall-stats}. 
\end{itemize}


\begin{table}[H]
    \centering
    \caption{Overall Statistics of the Generated Data. The number of environments used for each subset as well as the corresponding number of samples are reported. A breakdown of the number environments per obstacles is also presented in Table \ref{tab:envs} in Appendix \ref{app:env-stats}.}
    \label{tab:overall-stats}
    \begin{tabular}{@{}cccc}
      \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{\# of Envs}} & \multicolumn{1}{c}{\textbf{Single Goal}} & \multicolumn{1}{c}{\textbf{Multi-goal (No Constr./with Constr.)}} \\
      \hline
      \# \textbf{In-distribution (6x6 Grids)}  & \textbf{836} & \textbf{25,080} &  \textbf{83,600 (41,800/41,800)}\\
      \#   \textit{Train} & 668 & 16,032 &  53,440 (26,720/26,720) \\
      \#   \textit{Dev} & 668 & 2,004 &  6,680 (3,340/3,340) \\
      % \#   \textit{Test (Unseen Placements)} & 2,004 & 6,680 (3,340/3,340) \\
      \#   \textit{Test} & 168 & 5,040 & 16,800 (8,400/8,400) \\
            
      \hline
      \# \textbf{Out-of-distribution} & \textbf{375} & \textbf{12,000} &  \textbf{40,000 (20,000/20,000)} \\
      \#   \textit{7x7 Grids} & 125 & 3,750 &  12,500 (6,250/6,250) \\
      \#   \textit{5x5 Grids} & 125 & 3,750 & 12,500 (6,250/6,250)  \\
      \#   \textit{6-11 Obstacles} & 150 & 4,500 & 15,000 (7,500/7,500) \\
      \hline
    \end{tabular}

\end{table}



\textbf{Gold Plan Generation: } In order to generate the ground truths, we formulate the problem as a graph search problem. We use the A* path finding algorithm \citep{a_star} to find the optimal solutions for the single goal setting, while we combine this approach with a Traveling Salesman Problem (TSP) solver in order to provide solutions for the multi-goal setting. A more detailed description of the problem formulations is included in Appendix \ref{app:solutions}.

\textbf{Verbalizing into Natural Language: } The natural language descriptions of the queries are synthesized based on a number of templates, which can be found in Table \ref{tab:templates} in Appendix \ref{app:nl}


\subsection{Evaluation Metrics } 

We suggest the following metrics for evaluating the performance on the proposed tasks:

\textbf{Success Rate: } the percentage of generated action sequences that go from the intial location to the goal(s) while satisfying the constraints.

\textbf{Exact Match Accuracy: } the percentage of generated action sequences that are identical to the gold truth values.

\textbf{Optimal rate: } the percentage of generated paths that achieve the goal and are optimal. A path is optimal if reaches the goal(s) and avoids obstacles using the minimum possible number of actions.

\textbf{Feasible rate: } Generated paths that remain within the grid's boundaries and avoid obstacles, despite not reaching the goal.

\textbf{Distance to goal: } For the single world setting, it is computed as the length of the shortest path between the agent's final location according to the generated path and the desired goal. For the multi-goal setting, it is computed as the sum of optimal distances from the agent's location and the goals that were not reached. We penalize the paths that leave the grid by setting this metric to a large value (100).


==> iclr2023/sec_experiment.tex <==
\section{Experiments}\label{sec:experiment}




\subsection{Experimental Setup}

For our experiments, we chose to compare the performance achieved by fine-tuning T5 \citep{2020t5} and BART \citep{bart}, with the results achieved through in-context learning with GPT-4. We set up the large and base varieties of BART and T5 using the HuggingFace Transformers library \citep{wolf-etal-2020-transformers}. Training of the fine-tuned models was done using early stopping. We used four A100:40gb NVIDIA GPUs and per-device batch size of 16 to train all four models. 
For In-Context Learning experiments we access GPT-4 using OpenAI API; we set value of the temperature to 0. 


\subsection{Single Goal Results}

\begin{table}[t!]
\centering
\caption{Single-Goal Performance on the in-Distribution Test Set}
\label{tab:perf-sg}
\begin{tabular}{l c c c c c}
\hline
 & \textbf{Exact Match} & \textbf{Success Rate} & \textbf{Distance} & \textbf{Feasible} & \textbf{Optimal} \\
\hline
\textbf{In-Context Learning } &  &  &  &  & \\
\hspace{3mm} Naive few-shot (5) & 0.387 & 0.515 & 5.1 & 0.65 & 0.515 \\
\hspace{3mm} Naive few-shot (10) & 0.369 & 0.495 & 9.1 & 0.64 & 0.495 \\
\hspace{3mm} Naive few-shot (15) & 0.405 & 0.539 & 6.52 & 0.658 & 0.539 \\
\hspace{3mm} Actions+effects (5) & 0.529 & 0.779 & 0.0 & 0.779 & 0.779 \\
\hspace{3mm} CoT (5) & 0.6301 & 0.821 & 0.041 & 0.839 & 0.821 \\
\hspace{3mm} CoT + ReAct (5) & 0.6301 & \textbf{1.0} & 0.0 & \textbf{1.0} & 0.821 \\
\hline
\textbf{Fine-tuned Models } &  &  &  &  & \\
\hspace{3mm} BART-base & 0.7442 & 0.8061 & 4.405 & 0.9486 & 0.7966 \\
\hspace{3mm} BART-large & 0.921	& 0.9458 & 3.4873 & 0.9623 & 0.9392 \\
\hspace{3mm} T5-base & \textbf{0.973} & 0.98 & 2.014 & 0.982 & \textbf{0.979} \\
\hspace{3mm} T5-large & 0.923 & 0.978 & 2.5198 & 0.982 & 0.977 \\

\hline
\end{tabular}
\end{table}


The performance achieved on the in-distribution sets is presented in Table \ref{tab:perf-sg}. In this subsection, we discuss the different observations drawn from this table. 

\textbf{Increasing the number of few-shot exemplars aids GPT-4 in achieving the goal but does not assist in obstacle avoidance}. GPT-4's performance falls short when tasked with generating a complete path. Enhancing the quantity of few-shot examples yields minor improvements in exact match accuracy but fails to yield significant enhancements in success rates, especially when transitioning from 10 to 15 exemplars.  


Interestingly, while both 10 and 15 exemplars yield the same success rate, they tend to fail for different reasons. With 10 exemplars, the model often struggles to devise a plan that reaches the goal. In contrast, when prompted with 15 exemplars, failures primarily result from obstacles obstructing the predicted path. For instance, consider the task: \textit{'You are in a 6 by 6 world. There are obstacles that you have to avoid at: (0,4), (5,3) and (3,2). Go from (2,3) to (5,1)'}. Naive prompting with 10 examples generates the sequence \textit{'down down down left'} which not only encounters the obstacle at (5,3) but also falls one step short of the target. Conversely, prompting with 15 examples predicts the sequence \textit{'down down down left left'} which successfully reaches the goal but still encounters the same obstacle.

\textbf{Situated spatial information helps the model to make more informed decisions.} Actions and effects prompting shows promise as an approach. As illustrated in Table \ref{tab:perf-sg}, while exact match accuracy performance does not surpass that of naive prompting with 15 exemplars, the success rate exhibits significant improvement. This suggests that the model can generate better plans when it remains cognizant of its current location and does not need to plan multiple steps ahead. In other words, the model can decide to take an action that avoids an obstacle immediately after realizing that it is about to encounter one.

For the same test case mentioned above, this technique predicts: \textit{'Go down. You are now at (3,3). Go down. You are now at (4,3). Go left. You are now at (4,2). Go down. You are now at (5,2). Go left. You are now at (5,1). Hence, the action sequence is: down down left down left'}. By recognizing that it has reached (5,2), this method opts to turn left to circumvent the obstacle. However, it is not always successful in predicting encounters with obstacles. For example, in the task: \textit{'You are in a 6 by 6 world. There are obstacles that you have to avoid at: (1,4), (2,0), (4,5) and (2,5). Go from (0,4) to (2,3)'}, the generated sequence \textit{'down left down'} results in immediate contact with an obstacle after the first action.

\textbf{Reasoning can aid obstacle avoidance but falters for longer and more complex plans with numerous obstacles.} Our CoT approach offered significant gains in performance as can be seen in Table \ref{tab:perf-sg}. This indicates that GPT-4 may indeed possess a level of spatial reasoning capabilities and the ability to plan based on spatial information. For instance, it could easily generate a valid path for the test case failed by actions and effects prompting using the chain of thought: \textit{'(3,2) is 2 steps down and 2 steps to the right of (1,0). To avoid the obstacles at (1,1), (3,1), (1,3) and (3,3), I should move down first, then right. Therefore, my action sequence is: down down right right.'}. Nevertheless, when faced with examples involving more obstacles and cases where the goals are farther away, this technique also seemed to fail. 

For the task \textit{'You are in a 6 by 6 world. There are obstacles that you have to avoid at: (3,1), (5,1), (1,1), (3,3) and (1,3). Go from (1,0) to (3,2)'}, the chain of thought produced was: \textit{(3,2) is 2 steps down and 2 steps to the right of (1,0). To avoid the obstacles at (1,1), (3,1), (1,3) and (3,3), I should move down first, then right. Therefore, my action sequence is: down down right right.}, however, this reasoning chain was not helpful to the model, as following this path still leads to an obstacles. This type of reasoning also did not help with cases such as \textit{'You are in a 6 by 6 world. There are obstacles that you have to avoid at: (5,1), (0,0) and (1,0). Go from (0,5) to (4,0)' }, where the distance from the initial position to the goal is significant.

\textbf{GPT-4 is very effective at localized decision-making.} The shortcomings of CoT are overcome when this approach is combined with ReAct. Allowing the model to execute the valid portion of the plan and continuously improving the path by explicitly observing the effect of an action sequence through feedback from the environment, allows the model to generate one portion of the path at a time, removing the need for long term planning capabilities for this task. This approach achieves an impressive 100\% success rate. This points to the fact that GPT-4 does not struggle with spatial reasoning for our task but the difficulty comes from temporal aspect of our task. 

\textbf{Fine-tuning can be an effective approach.} As we can see from Table \ref{tab:perf-sg}, BART-Large, as well as both varieties of T5 achieve a good performance, with the T5 model achieving a success rate of 98\%.  Fine-tuned models' performance appears to be impressive at first glance, achieving close results on both environments seen during training with novel placements of initial and goal locations and on completely novel environments as illustrated in Figure \ref{fig:seenvunseen}. However, these models are known to fail when at generalizing to out-of-distribution examples; we evaluate this hypothesis next.

An interesting observation to be made is that while the vast majority of failures produced by GPT-4 are due to the model running to an obstacle, with fine-tuned a model a large number of errors were to the model avoiding all obstacles but landing at a location on the grid other than the goal, as evidenced by the higher values for the feasible rate and the distance metrics. 

\textbf{Fine-tuned models can generalize to simpler grids but not to more complex ones.} We illustrate the performance on out-of-distribution test sets of both the fine-tuned models and the best performing in-context learning techniques in Figure \ref{fig:ood-sg}. Interestingly, the fine-tuned models were able to generalize well to the 5x5 environments. We hypothesize that this is because 5x5 environments are inherently part of the 6x6 environments encountered in training. For the 7x7 environments, however, all of the fine-tuned models failed to perform well. This highlights out-of-distribution generalization as an important limitation of fine-tuned models.

\textbf{GPT-4 can generalize to larger grids but struggles when more obstacles are involved.} GPT-4 prompted with ReAct achieved near-perfect performance; this goes along with the hypothesis that larger auto-regressive models such as GPT-4 are better at out-of-distribution generalization when compared to their smaller fine-tuned counterparts. However, GPT-4 still struggled when faced with more obstacles than the ones seen in the the few shot exemplars, with ReAct prompting performing slightly worse than both T5 models. However, we believe this can be improved by allowing more than three trials for ReAct to attempt to correct its path. 

\begin{figure}[tb]

    \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\textwidth]{iclr2023/figures/seen.png}
        \caption{Unseen Placements}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\textwidth]{iclr2023/figures/unseen.png}
        \caption{Unseen Environments}
    \end{subfigure}
    \caption{Fine-tuned Models' Performance on the Single Goal Setting}
    \label{fig:seenvunseen}
\end{figure}

\begin{figure}[tb]
    \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\textwidth]{iclr2023/figures/5x5worlds.png}
        \caption{Performance on 5x5 Environments}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\textwidth]{iclr2023/figures/7x7worlds.png}
        \caption{Performance on 7x7 Environments}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \hspace{0.25\textwidth}
        \includegraphics[width=0.5\textwidth]{iclr2023/figures/moreobsts.png}
        \captionsetup{justification=centering} 
        \caption{Performance on Obstacles 6-11}
    \end{subfigure}
    \caption{Out-of-Distribution Performance for the Single-Goal Setting}
    \label{fig:ood-sg}
\end{figure}

\subsection{Scaling up to Multiple Goals}

    Next, we look at how the best performing models on the single-goal setting scale-up to the multiple-goals. Namely, We evaluate end-to-end planning using T5, as well as how CoT+ReAct performs when multiple goals are to be visited.

    \textbf{Fine-tuned models can scale up to multi-goal path planning scenarios. } Table \ref{tab:multigoal-res} shows the performance of the different LLMs on the in-distribution test set. While the exact match accuracy of the model is much lower compared to the single-goal setting, the value of the success rate is very close. The lower exact match values, particularly for the case with no constraints, is due to the fact that with this task, a larger number of paths can be taken to reach the goal.
    
    As far as out-of-distribution generalization is concerned, as illustrated in Figure \ref{fig:ood-mg}, while the models are still able to generalize well on the 5x5 environments, the gap between the in-distribution and out-of-distribution performance in this setting is much larger.

    \textbf{CoT+ReAct is not as successful when multiple goals are involved.} As we can see from Table \ref{tab:multigoal-res}, CoT+ReAct fails to achieve the same success from the single goal setting in a multi-goal context.  The vast majority of failures occur with tasks involving environments involving 4 or 5 obstacles and scenarios involving six goals.

    \begin{table}[H]
    \centering
    \caption{Multi-Goal Performance on Unseen Environments}
    \label{tab:multigoal-res}
    \begin{tabular}{l c c c c c}
    \hline
     & \textbf{Exact Match} & \textbf{Success Rate} & \textbf{Distance} & \textbf{Feasible} & \textbf{Optimal} \\
    \hline
    \textbf{No Constraints} &   &  &  &  & \\
    \hspace{3mm} T5-base & 0.543 & 0.969 & 0.652 & 0.982 & 0.796 \\
    \hspace{3mm} Chained CoT + ReAct & 0.083 & 0.845 & 0.535 & 0.928 & 0.309 \\
    \hline
    \textbf{With Constraints } &  &  &  &  & \\
    \hspace{3mm} T5-base & 0.781 & 0.971 & 0.683 & 0.979 & 0.894  \\
    \hspace{3mm} Chained CoT + ReAct & 0.120 & 0.831 & 0.675 & 0.922 & 0.253  \\
    
    \hline
    \end{tabular}
    \end{table}

\begin{figure}[H]
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{iclr2023/figures/multi-5x5.png}
        \caption{Performance on 5x5 Environments}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{iclr2023/figures/multi-7x7.png}
        \caption{Performance on 7x7 Environments}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \hspace{0.25\textwidth}
        \includegraphics[width=0.45\textwidth]{iclr2023/figures/multi-moreobsts.png}
        \captionsetup{justification=centering} % Center the caption
        \caption{Performance on Obstacles 6-11}
    \end{subfigure}
    \caption{Out-of-Distribution Performance for the Multi-Goal Setting (T5-base)}
    \label{fig:ood-mg}
\end{figure}


    



\subsection{Discussion and Analysis}\label{sec:finegrain}

    
    \textbf{Does the performance depend on the number of obstacles?} Figures \ref{fig:numofobsts} and \ref{fig:cot-numofobsts} point to the fact that adding more obstacles can adversely affect performance. However, while the overall performance of CoT prompting is lower than that of T5-base, it seems to fair better when more obstacles are involved. The superior performance of T5 on the obstacles 6-11 test set seems to be largely attributed to its good performance on environments with 6 obstacles, as prompting with CoT outperforms T5 on environments with a number obstacles ranging between 7 and 11; pointing to the fact that GPT-4 is indeed more proficient at out-of-distribution generalization in comparison to fine-tuned models such as T5. 
    
    \textbf{Is it harder to reach distant goals?} Looking at Figure \ref{fig:pathlength}, it is evident that T5's performance starts to decline as the ground truth path length increases. In other words, T5 encounters difficulties in finding solutions for reaching distant goals, resulting in a success rate of 0 for goals beyond a distance of 10 steps. A similar trend can be observed for GPT-4 when prompted with CoT, as depicted in Figure \ref{fig:cot-pathlen}. However, it is worth noting that GPT-4 appears to face even greater challenges in achieving distant targets. This suggests that while GPT-4, with the assistance of CoT, exhibits enhanced robustness in out-of-distribution generalization compared to smaller fine-tuned models, it is less successful at long-term planning.

    \begin{figure}[tb]
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{iclr2023/figures/pathslen.png}
        \caption{T5-Base performance as a function of the path length}
        \label{fig:pathlength}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{iclr2023/figures/obsts_.png}
        \caption{T5-Base performance as a function of the number of obstacles}
        \label{fig:numofobsts}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{iclr2023/figures/cot-pathlen.png}
        \caption{CoT prompting performance as a function of the the path length}
        \label{fig:cot-pathlen}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{iclr2023/figures/num-obsts.png}
        \caption{CoT prompting performance as a function of the number of obstacles}
        \label{fig:cot-numofobsts}
    \end{subfigure}
    \caption{Fine-Grained Performance of the Best Performing Finetuned Model (T5-base) and CoT prompting (single goal).}
    
\end{figure}
    
    \textbf{Does the action space matter?} Another question we ask is whether representing the task differently affects the models' performance. To explore this, we propose an alternative setting where we constrain the agent's movement to the direction it is facing. In this case, the action space comprises three instances: turn left, turn right, and move forward. We assume the agent always starts facing south. 
    
    We evaluate the performance of the t5-base model using this representation in the single-goal setting and present the results in Table \ref{tab:direction}. With this representation, we observe a slight decrease in performance, indicating that the manner in which we present the task to the models is an important consideration. Due to cost and time limitations, we did not conduct all the experiments considered in this work using this representation. However, we have included solutions based on this representation in our benchmark, which will be made publicly available for use by other researchers who wish to further explore this question.
        \begin{table}[H]
    \centering
    \caption{T5-base performance considering agent direction}
    \label{tab:direction}
    \begin{tabular}{l c c c c c}
    \hline
    \textbf{Test Set} & \textbf{Exact Match} & \textbf{Success Rate} & \textbf{Distance} & \textbf{Feasible} & \textbf{Optimal} \\
    \hline
    Unseen Placements &  0.967 & 0.967 & 3.02 & 0.975 & 0.965 \\
    Unseen Environments & 0.966 & 0.968 & 2.11 & 0.976 & 0.967 \\
    5x5 Environments & 0.954 & 0.954 & 3.48 & 0.962 & 0.954 \\
    7x7 Environments & 0.527 & 0.546 & 0.885 & 0.893 & 0.533 \\
    6-11 Obstacles & 0.749 & 0.749 & 18.11 & 0.775 & 0.754  \\

    
    
    \hline
    \end{tabular}
    \end{table} 

    \textbf{Is GPT-4 able to find the optimal path?} An interesting observation drawn from Table \ref{tab:perf-sg} is that whenever any of the prompting techniques were able to find a solution without the need for correction in the single-goal setting, the solution was also optimal, despite the need for an optimal solution not being mentioned in the prompt. However, we noticed a significant drop in this metric when scaling up to multiple goals. 
    
    The ordering generated in our hierarchical approach was not always optimal. Hence, we conduct an additional experiment where we specifically prompt the models for the optimal order. We use A* search to compute the optimal distance between every two subsequent locations in the generated ordering and evaluate the optimality of the plan. 
    
    From Table \ref{tab:optimal-ordering}, we notice that explicitly prompting the models for the optimal does not offer any improvements on this metric. In fact, curiously, for the case of examples involving constraints, the percentange of optimal orderings drops. Achieving the optimal ordering requires the model to implicitly solve an instance of TSP. Doing this requires significant temporal reasoning capabilities. Exploring ways to improve on this metric for the multi-goal setting can be an interesting avenue of research to be explored as part of future work.

    \begin{table}[H]
    \centering
    \caption{Results when Prompting for the Optimal Order}
    \label{tab:optimal-ordering}
    \begin{tabular}{l c c c c c}
    \hline
     &  \textbf{Constraints Satisfied} & \textbf{Optimal Ordering} \\
    \hline
    \textbf{No Constraints} &  &  \\
    \hspace{3mm} Prompting w/ no Optimality & - & 0.43 \\
    \hspace{3mm} Prompting w/ Optimality & - & 0.43 \\
    \hline
    \textbf{With Constraints } &  & \\
    \hspace{3mm} Prompting w/ no Optimality & 1.0 & 0.42 \\
    \hspace{3mm} Prompting w/ Optimality & 1.0 & 0.36 \\
    
    \hline
    \end{tabular}
    \end{table}

    \textbf{Does GPT-4 struggle more with space or time?} The overall results highlight that GPT-4 exhibits impressive spatial reasoning capabilities. This can be particularly seen by the performance gains offered by the actions and effects prompting when compared to naive prompting, which indicates that providing situated knowledge at each step does help the model make better decisions at each step, however, they fail at planning few steps ahead. The impressive performance of ReAct also seems to point to the same conclusions as substantial gains in performance can be offered but explicitly informing the model of its current location and only expecting it to plan a few-steps ahead.

    \textbf{Time and Cost Considerations: } Table \ref{tab:cost} in Appendix \ref{time-cost} provides the average cost and inference time per sample for all approaches. ReAct prompting has an average cost that far exceeds all other methods. This is due to the nature of the technique as it requires repeatedly making API in attempt to adjust the predicted path. This makes this approach too costly for real-world applications that require long distance navigation and many corrections. It is, hence, imperative to find approaches that can perform similarly to this technique at a lower cost.

    

    







==> iclr2023/sec_experiment2/additional_analysis.tex <==
\section{Discussion and Analysis}

\textbf{Does the performance depend on the number of obstacles?} Figure \ref{fig:numofobsts} points to the fact that adding more obstacles can adversely affect performance. Nevertheless, T5-base appears to fair much better than CoT. While prompting the model the model to think step-by-step does indeed allow it to make better decisions, it fails when there is multiple obstacles to be avoided. This could indicate that while GPT-4 possesses a basic level of spatial reasoning, it struggles to utilize this skill for complex reasoning chains. 

% \begin{figure}[H]
% \begin{subfigure}{0.45\textwidth}
%    \includegraphics[width=\textwidth]{iclr2023/figures/per_obst_stats.pdf}
%    \caption{T5-Base performance as a function of the number of obstacles (Single-Goal)}
%    \label{fig:numofobsts-t5}
% \end{subfigure}
% \end{figure}

\begin{wrapfigure}{R}{0.35\textwidth} 
  \centering
  \includegraphics[width=0.35\textwidth]{iclr2023/figures/per_obst_stats.pdf}
  \caption{The success rate of T5-based and GPT-4 with CoT in single-goal setting.}
  \label{fig:numofobsts}
\end{wrapfigure}

    
\textbf{Is it harder to reach distant goals?} Looking at Figure \ref{fig:t5_path_len}, it is evident that T5's performance starts to decline as the ground truth path length increases. In other words, T5 encounters difficulties in finding solutions for reaching distant goals. A similar trend can be observed for GPT-4 when prompted with Chained CoT+React, as depicted in Figure \ref{fig:hierarch_path_len}. However, it is worth noting that GPT-4 appears to face even greater challenges in achieving distant targets. This suggests that GPT-4 is less successful at long-term planning. This approach's failure is particularly apparent in terms of optimal rate, further supporting the claim that while ReAct can improve the models ability to reach the desired destination through path correction, it still fails to improve the temporal reasoning aspect of our task, as finding the optimal path requires planning on longer horizons.

% 
\begin{figure}[H]
% % \begin{subfigure}{0.45\textwidth}
% %     \includegraphics[width=\textwidth]{iclr2023/figures/length-stats.pdf}
% %     \caption{T5-Base performance as a function of the path length}
% %     \label{fig:pathlength}
% % \end{subfigure}
% %\hfill
% %\begin{subfigure}{0.4\textwidth}
% %    \includegraphics[width=\textwidth]{iclr2023/figures/more_obsts_t5.pdf}
% %    \caption{T5-Base performance as a function of the number of obstacles}
% %    \label{fig:numofobsts}

\centering
\begin{subfigure}{0.35\textwidth}
     \includegraphics[width=\textwidth]{iclr2023/figures/t5_out_stats.pdf}
     \caption{T5-Base performance as a function of the path length}
     \label{fig:t5_path_len}
\end{subfigure}
\hspace{14mm}
\begin{subfigure}{0.35\textwidth}
     \includegraphics[width=\textwidth]{iclr2023/figures/cot_len_stats.pdf}
     \caption{Chained CoT+React performance as a function of the path length}
     \label{fig:hierarch_path_len}
\end{subfigure}
% \begin{subfigure}{0.45\textwidth}
% %     \includegraphics[width=\textwidth]{iclr2023/figures/path-len-cot.pdf}
% %     \caption{CoT prompting performance as a function of the the path length}
% %     \label{fig:cot-pathlen}
% \end{subfigure}
% %\hfill
% % \begin{subfigure}{0.4\textwidth}
% %     \includegraphics[width=\textwidth]{iclr2023/figures/per-obst-cot.pdf}
% %     \caption{CoT prompting performance as a function of the number of obstacles}
% %     \label{fig:cot-numofobsts}
% % \end{subfigure}
\caption{Performance of the Best Performing Finetuned Model (T5-base) and Chained CoT+ReAct (multi-goal) based on path length of the ground truth plan.}

\end{figure}

\textbf{Is GPT-4 able to find the optimal path?} An interesting observation drawn from Table \ref{tab:perf-sg} is that whenever any of the prompting techniques were able to find a solution without the need for correction in the single-goal setting, the solution was also optimal, despite the need for an optimal solution not being mentioned in the prompt. However, we noticed a significant drop in this metric when scaling up to multiple goals.

The ordering generated in our hierarchical approach was not always optimal. Hence, we conduct an additional experiment where we specifically prompt the models for the optimal order. We use A* search to compute the optimal distance between every two subsequent locations in the generated ordering and evaluate the optimality of the plan. 

From Table \ref{tab:optimal-ordering}, we notice that explicitly prompting the models for the optimal does indeed offer slight improvements on this metric. However, the overall performance is still quite low. Achieving the optimal ordering requires the model to implicitly solve an instance of TSP. Doing this requires significant temporal reasoning capabilities. Exploring ways to improve on this metric for the multi-goal setting can be an interesting avenue of research to be explored as part of future work. Recent work \citep{yang2023large} has proposed methods to utilize LLMs as optimizers, which can be a promising avenue of research. We believe that our benchmark can be a great resource for researchers wishing to explore this idea.



\begin{wraptable}{R}{0.55\textwidth}
\centering


\caption{Results of GPT-4 when prompted for optimal order or not.}

\resizebox{\linewidth}{!}{
\begin{tabular}{l c c c c c}
\hline
 &  \textbf{Constraints Satisfied} & \textbf{Optimal Ordering} \\
\hline
\textbf{No Constraints} &  &  \\
\hspace{3mm} Prompting w/ no Optimality & - & 0.47 \\
\hspace{3mm} Prompting w/ Optimality & - & 0.51 \\
\hline
\textbf{With Constraints } &  & \\
\hspace{3mm} Prompting w/ no Optimality & 1.0 & 0.52\\
\hspace{3mm} Prompting w/ Optimality & 1.0 & 0.56 \\

\hline
\end{tabular}}\label{tab:optimal-ordering}
\end{wraptable}

\textbf{Does GPT-4 struggle more with space or time?} The overall results highlight that GPT-4 exhibits some level of spatial reasoning capabilities. This can be particularly seen by the performance gains offered by the actions and effects prompting when compared to naive prompting, which indicates that providing situated knowledge at each step does help the model make better decisions, however, they fail at planning many steps ahead. The impressive performance of ReAct also seems to point to the same conclusions as substantial gains in performance can be offered by explicitly informing the model of its current location and only expecting it to plan a few actions ahead.

\textbf{Cost Considerations: } Table \ref{tab:cost} in Appendix \ref{time-cost} provides the average cost per sample for all approaches. ReAct prompting has an average cost that far exceeds all other methods. This is due to the nature of the technique as it requires repeatedly making API in attempt to adjust the predicted path. This makes this approach too costly for real-world applications that require long distance navigation and many corrections. It is, hence, imperative to find approaches that can perform similarly to this technique at a lower cost.

==> iclr2023/sec_intro.tex <==
\section{Introduction}\label{sec:intro}

Large Language Models (LLMs) have ignited a revolution in Artificial Intelligence and Natural Language Processing. Transformer-based models (e.g., \citep{NIPS2017_attn, radford2018improving, liu2019roberta, devlin-etal-2019-bert, 2020t5, bart}), leveraging self-attention mechanisms, have achieved remarkable performance across diverse natural language tasks. These models shattered expectations by scaling hyperparameters, leading to groundbreaking models like GPT-3 \citep{brownGPT3} and its successors, GPT-3.5 \citep{chatgpt_2023} and GPT-4 \citep{openai2023gpt4}, each boasting hundreds of billions of parameters. They have astounded the world with their linguistic and reasoning capabilities, sparking vigorous debates among researchers about their role in advancing Artificial General Intelligence (AGI) \citep{bubeck2023sparks, marcus2023sentence, butlin2023consciousness}.

Spatial-temporal reasoning is a fundamental aspect of human intelligence. Humans possess the ability to seamlessly integrate spatial information from their surroundings into their decision-making processes, enabling them to make informed choices and take appropriate actions based on their spatial awareness. LLMs, trained solely on textual data, have been criticized by many for not possessing this skill \citep{agrawal2023llms, chen_arkin_zhang_roy_fan_2023, bubeck2023sparks}. In this work, we attempt to analyze this skill in LLMs and whether they can be grounded to perform actions in a simplistic environment. To this end, we look at whether LLMs can perform well on a task that requires reasoning about both a temporal and spatial aspect: path planning. 

Various benchmarks have been proposed to ground language into an environment in order to to test situated planning skills. For instance, \cite{Ruis2020ABF} propose gSCAN, a benchmark for assessing compositional generalization in situated language understanding. \cite{wu2021reascan} extend this benchmark by including commands that necessitate compositional language understanding and more complex reasoning about the different entities. While both of these datasets can offer great insights into the spatial reasoning capabilities of LLMs, very little planning is required from the models as the tasks are relatively simple once the natural language command is understood. Furthermore, as the datasets are multi-modal, often times, the performance of the LLMs can only be as good as the computer vision module used to verbalize the environments into natural language. This is also a shortcoming of a number of other benchmarks that have been widely used for motion and task planning, such as STAR \citep{wu2021star} and ALFRED \citep{ALFRED20}, the environments used in these datasets are also very complex, making it hard to control for the distribution of the samples and reliably control for different variables, which may offer additional insights into LLMs performance on the task.

To address these shortcomings, we propose \textbf{P}ath \textbf{P}lanning from \textbf{N}atural \textbf{L}anguage (PPNL), a benchmark for assessing LMs as end-to-end path planners. We generate a synthetic dataset of over 160,000 samples, consisting of queries requiring an agent to navigate from an initial location to a set of goal locations while satisfying some constraints. We assess the performance of different prompting techniques with GPT-4. To this end, we experiment with four different designs: (1) \textit{naive few-shot prompting}, where we provide few shot exemplars of task descriptions and the corresponding end-to-end plans, (2) \textit{actions and effects prompting}, where we prompt the model to reason about keep track of what its current location is after performing each action, (3) \textit{Chain-of-Thought Reasoning} \cite{CoT2022} by requiring the model to reason about what steps should be taken and how to avoid obstacles, and extend this idea using (4) \textit{ReAct} \cite{yao2023react} where the model can continuously correct its path based on feedback from the environment.  Finally, we look at how GPT-4 fares on this task when compared to smaller fine-tuned models, namely T5 \citep{2020t5} and BART \citep{bart}.

Our findings suggest that GPT-4 demonstrates strong spatial reasoning abilities, as evidenced by the significant performance improvements achieved through actions and effects prompting compared to naive prompting, suggesting that providing the model with situated knowledge at each step helps it make better immediate decisions. However, GPT-4 falls short in terms of long-term planning. The remarkable performance of ReAct further underscores this limitation, indicating that explicitly informing the model of its current location and expecting it to plan only a few steps ahead can lead to substantial performance gains. 

Our proposed dataset can be a useful resource for researchers from the realms of robotics and motion planning as well as natural language processing. We provide our dataset as well as the code to synthesize it, for anyone wishing to extend it and generate more settings and scenarios than the ones included in this analysis. This can serve as a simple yet effective benchmark for evaluating path planning capabilities through natural language. Our analysis of various LLMs' performance on this task can also offer meaningful insights into the spatial-temporal reasoning capabilities of LLMs. 

==> iclr2023/sec_methods.tex <==
\section{Methodologies}

\begin{figure}[tb]
  \centering
  \includegraphics[width=\linewidth]{iclr2023/figures/figure2.png}
  \caption{Overview of the methods explored for In-Context Learning.}
  \label{fig:label}
\end{figure}

\subsection{Methods Considered}

We experiment with a variety of prompts for in-context learning; we wanted to evaluate the extent to which GPT-4 can perform spatial-temporal reasoning within the context of path planning.  All in-context learning experiments were performed between August and September of 2023. The prompts used for these experiments are presented in Appendix \ref{prompts}.

Due to the limited resources at our disposal, all in-context learning experiments were only run on a a subset of the test sets, consisting of one randomly drawn placement from each environment. In other words, we sample one example from each environment in Table \ref{tab:envs}; as such, in total, we ended up with a total of 168 examples for the in-distribution test set, 125 for generalization to 7x7 environments, 125 for 5x5 environments and 150 for 6-11 Obstacles. However, we use the full datasets for the fine-tuning experiments.

\textbf{Naive Prompting:} The first case we consider is in-context learning through prompting using only the set of actions required to reach the desired goals. For this case, we consider prompts with few-shot exemplars ranging between 5 and 15. 

\textbf{Prompting with Actions and their Effects: } We also evaluate whether prompting the models with the effect of each action (i.e. the current state after performing the action) helps better guide the model towards a solution. In other words, we look at whether prompting the model to infer the effect of the each action taken can allow the model to take better decisions. 

\textbf{Chain of Thought Prompting: } Furthermore, we consider Chain-of-Thought (CoT) reasoning \citep{CoT2022}, an approach that has proven to be effective across a wide-range of tasks. We use this approach to prompt the model to reason about: (1) how far the goal is from the start location, and (2) which actions to take to avoid any obstacles that may fall on the path from the initial placement to the goal.

\textbf{ReAct Prompting:} In an attempt to push the two previous approaches to their fullest, we extend CoT with the Reason + Act (ReAct) \citep{yao2023react} technique in order to ground the model to the environments and allow for corrections through continuous feedback. In this case, we allow the GPT-4 to generate a new trajectory whenever performing the next action in a predicted sequence leads to invalid path. In this case, the model is prompted to generate a path from its current location (i.e. one step before running into an obstacle or falling outside the grid) to the goal location. We allow up to three trials, after which, if the agent still hasn't reached the goal using the provided sequences, we mark the case as a failure. 

\textbf{Fine-tuning:} We also look at whether smaller pre-trained LMs can outperform GPT-4 if repurposed for the task through fine-tuning. 
    
\textbf{Chained CoT + ReAct: }  For GPT-4 in a multi-goal setting, we experiment with a hierarchical approach, where we first prompt the model to generate an ordering in which the locations are to be visited. Then GPT-4 with CoT+ReAct is run to find a path between each subsequent locations, in a similar fashion to the single goal setting. 

\textbf{Out-of-distribution Generalization: } Next, we look at whether the LMs can solve the problem on environments of different properties than the ones used for training.

\subsection{Evaluation Metrics } 

We suggest the following metrics for evaluating the performance on the proposed tasks:

\textbf{Success Rate: } the percentage of generated action sequences that go from the intial location to the goal(s) while satisfying the constraints.

\textbf{Exact Match Accuracy: } the percentage of generated action sequences that are identical to the gold truth values.

\textbf{Optimal rate: } the percentage of generated paths that achieve the goal and are optimal. A path is optimal if reaches the goal(s) and avoids obstacles using the minimum possible number of actions.

\textbf{Feasible rate: } Generated paths that remain within the grid's boundaries and avoid obstacles, despite not reaching the goal.

\textbf{Distance to goal: } For the single world setting, it is computed as the length of the shortest path between the agent's final location according to the generated path and the desired goal. For the multi-goal setting, it is computed as the sum of optimal distances from the agent's location and the goals that were not reached. We penalize the paths that leave the grid by setting this metric to a large value (100).


==> iclr2023/sec_results_fewshot.tex <==
\section{Results for Few-shot LLMs}\label{sec:few-shot}

==> iclr2023/sec_results_finetune.tex <==
\section{Results for Fine-tuned LLMs}\label{sec:fine-tune}
